Neural Extractive Text Summarization with Syntactic Compression

Recent neural network approaches to summarization are largely either selection-based extraction or generation-based abstraction. In this work, we present a neural model for single-document summarization based on joint extraction and syntactic compression. Our model chooses sentences from the document, identifies possible compressions based on constituency parses, and scores those compressions with a neural model to produce the final summary. For learning, we construct oracle extractive-compressive summaries, then learn both of our components jointly with this supervision. Experimental results on the CNN/Daily Mail and New York Times datasets show that our model achieves strong performance (comparable to state-of-the-art systems) as evaluated by ROUGE. Moreover, our approach outperforms an off-the-shelf compression module, and human and manual evaluation shows that our model's output generally remains grammatical.

==> tab-seurvey.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{c|cccc}
\toprule
Node Type & \multicolumn{1}{l}{Len} & \multicolumn{1}{l}{\% of comps} & \multicolumn{1}{l}{Oracle comp \%}  \\
\midrule
PP        & 5.7                      & 39\%                          & 67\%                          \\
JJ        & 1.0                      & 19\%                          & 84\%                          \\
SBAR      & 12.1                      & 11\%                          & 59\%                          \\
ADVP      & 1.3                      & 7\%                           & 91\%                   \\\bottomrule      
\end{tabular}
\caption{Statistics of compression options on CNN. We show the top four constituency types that are compressible, along with the average length, the fraction of available compressions it accounts for, and how frequently the oracle says to compress these constituents.}
 \label{tb:surv-bf}
\end{table}

\begin{table}[t]
\centering
\small
\renewcommand{\tabcolsep}{1.8mm}
\begin{tabular}{c|cccc}\toprule
Node Type & \multicolumn{1}{l}{Len} & \multicolumn{1}{l}{\% of comps} & \multicolumn{1}{l}{Comp Acc} & \multicolumn{1}{l}{Dedup}  \\\midrule
JJ        & 1.0                           & 34\%                           & 72\%                         & 30\%                        \\
PP        & 3.4                           & 26\%                           & 47\%                         & 72\%                        \\
ADVP      & 1.4                           & 17\%                           & 79\%                         & 17\%                        \\
PRN       & 2.2                           & 6\%                            & 80\%                         & 5\%                         \\\bottomrule 
\end{tabular}
\caption{The compressions actually used by our model on CNN; average lengths and the fraction of that constituency type among compressions taken by our model. Comp Acc indicates how frequently that compression was taken by the oracle; note that error, especially keeping constituents that we shouldn't, may have minimal impact on summary quality.  Dedup indicates the percentage of chosen compressions which arise from deduplication as opposed to model prediction. Many PPs are removed in this process contrary to what the oracle states.}
  \label{tb:surv-af}
\end{table}


==> tab_exp_cnndm.tex <==


\begin{table*}[t!]
\centering
\small
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Model}       & \multicolumn{3}{c|}{CNNDM} & \multicolumn{3}{c|}{CNN} & \multicolumn{3}{c}{DM}  \\
                                                           & R-1  & R-2  & R-L         & R-1  & R-2  & R-L       & R-1  & R-2  & R-L       \\
                                                           \midrule
% Lead PointGenCov \citep{See_Get_2017}                                               & 40.3 & 17.7 & 36.6        & -- & -- & -- & -- &-- & --   \\
%  Lead Refresh \citep{Narayan_Ranking_2018}                                               & 39.6 & 17.7 & 36.2        & 29.1 & 11.1 & 25.9      & 40.7 & 18.3 & 37.2      \\\
% Lead Neusum \citep{Zhou_Neural_2018}                                                & 40.2 & 17.7 & 36.5        &  --    &  --    & --          &  --    &   --   &    --       \\
% Lead LatSum \citep{Zhang_Neural_2018}                                              & 40.3 & 17.7 & 36.6      &  --    &  --    & --          &  --    &   --   &    --              \\
% Lead BanditSum \citep{Dong_BanditSum_2018}                                             & 40.0 & 17.5 & 36.2        & 28.8 & 11.0 & 25.5      & 41.2 & 18.2 & 37.3      \\
Lead  (Ours)         & 40.3 & 17.6 & 36.4        & 29.1 & 11.1 & 25.8      & 41.3 & 18.2 & 37.4      \\
\midrule
%Refresh   & 40.0 & 18.2 & 36.6        & 30.4 & 11.7 & 26.9      & 41.0 & 18.8 & 37.7      \\
Refresh*     \citep{Narayan_Ranking_2018}              & 40.0 & 18.1 & 36.6        & 30.3 & \textbf{11.6} & 26.9      & 41.0 & 18.8 & 37.7      \\
NeuSum  & \textbf{41.6} & \textbf{19.0} & 38.0       &  --    &  --    & --          &  --    &   --   &    --        \\
%LatSum                                                     & 41.0 & 18.8 & 37.5       &  --    &  --    & --          &  --    &   --   &    --       \\
LatSum*  \citep{Zhang_Neural_2018}      & 41.0 & 18.8 & 37.4        & 28.8 & 11.5 & 25.4      & \textbf{42.3} & \textbf{19.5} & \textbf{38.6}      \\
LatSum w/ Compression                                                  & 36.7 & 15.4 & 34.3       &  --    &  --    & --          &  --    &   --   &    --          \\
BanditSum                                                  & 41.5 & 18.7 & 37.6        & \textbf{30.7} & \textbf{11.6} & \textbf{27.4}      & 42.1 & 18.9 & 38.3      \\
%  PointGenCov     & 39.5 & 17.3 & 36.4        &  --    &  --    & --          &  --    &   --   &    --            \\
CBDec \citep{Jiang_Closed_2018}                                           & 40.7 & 17.9 & 37.1      &  --    &  --    & --          &  --    &   --   &    --                  \\
 FARS \citep{Chen_Fast_2018}      & 40.9 & 17.8 & \textbf{38.5}        &  --    &  --    & --          &  --    &   --   &    --            \\
%   \citep{Pasunuru_Multi_2018}              & 41.5 & 18.7 & 37.8     &  --    &  --    & --          &  --    &   --   &    --                  \\
% NeuSum*                                                    &      &      &             &      &      &           &      &      &           \\
\midrule
\textsc{LeadDedup}                                      & 40.5 & 17.4 & 36.5        & 29.7 & 10.9 & 26.2      & 41.7 & 18.1 & 37.7      \\
\textsc{LeadComp}                                                & 40.8 & 17.4 & 36.8        & 30.6 & 10.8 & 27.2      & 42.0 & 18.0 & 37.9      \\
\textsc{Extraction}                                               & 40.7 & 18.0 & 36.8        & 30.3 & 11.0 & 26.5      & 41.7 & 18.9 & 38.0      \\
\textsc{JECS}                                                  & \textbf{41.7} & \textbf{18.5} &\textbf{ 37.9 }       & \textbf{32.7} & \textbf{12.2} & \textbf{29.0}      &\textbf{ 42.7} & \textbf{19.2} &\textbf{ 38.8}     \\
\bottomrule
\end{tabular}
\caption{Experimental results on the test sets of CNN and DM. We report ROUGE F1 of models trained and tested on CNN/DM together as well as separately. * indicates models evaluates with our own ROUGE metrics. Our model outperforms our extractive model and lead-based baselines, as well as prior work. Gains are more pronounced on CNN because this dataset features shorter, more compressed reference summaries.
}
  \label{tb:cnndm}
\end{table*}

==> tab_oracle_upper.tex <==

\begin{table}[t]
  \centering
  \small
  \begin{tabular}{c|ccc}
  \toprule
  \multirow{1}{*}{Oracle} 
%   &  \multicolumn{4}{c}{PTB}
     & CNN & DM & NYT   \\
\midrule
Extraction	&	32.2	&	42.7	&45.9 \\
Extraction + Compression	&	36.9	&	46.1	&50.0 \\
\bottomrule
  \end{tabular}
  \caption{ROUGE-1 F$_1$ values between extractive oracle and joint extractive and compressive oracle described in the text. On each dataset, the extractive and compressive oracle outperforms the extractive oracle by a substantial margin.
  }
  \label{tb:oracle_compare}
\end{table}

==> tab_surv_bf.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{c|cccc}
\toprule
Node Type & \multicolumn{1}{l}{Len} & \multicolumn{1}{l}{\% of comps} & \multicolumn{1}{l}{Oracle comp \%}  \\
\midrule
PP        & 5.7                      & 39\%                          & 67\%                          \\
JJ        & 1.0                      & 19\%                          & 84\%                          \\
SBAR      & 12.1                      & 11\%                          & 59\%                          \\
ADVP      & 1.3                      & 7\%                           & 91\%                   \\\bottomrule      
\end{tabular}
\caption{Statistics of compression options on CNN. We show the top four constituency types that are compressible, along with the average length, the fraction of available compressions it accounts for, and how frequently the oracle says to compress these constituents.}
 \label{tb:surv-bf}
\end{table}
